MVP-Bench: Can Large Vision--Language Models Conduct Multi-level Visual Perception Like Humans?

Humans perform visual perception at multiple levels, including low-level object recognition and high-level semantic interpretation such as behavior understanding. Subtle differences in low-level details can lead to substantial changes in high-level perception. For example, substituting the shopping bag held by a person with a gun suggests violent behavior, implying criminal or violent activity. Despite significant advancements in various multimodal tasks, Large Visual-Language Models (LVLMs) remain unexplored in their capabilities to conduct such multi-level visual perceptions. To investigate the perception gap between LVLMs and humans, we introduce MVP-Bench, the first visual-language benchmark systematically evaluating both low- and high-level visual perception of LVLMs. We construct MVP-Bench across natural and synthetic images to investigate how manipulated content influences model perception. Using MVP-Bench, we diagnose the visual perception of 10 open-source and 2 closed-source LVLMs, showing that high-level perception tasks significantly challenge existing LVLMs. The state-of-the-art GPT-4o only achieves an accuracy of $56\%$ on Yes/No questions, compared with $74\%$ in low-level scenarios. Furthermore, the performance gap between natural and manipulated images indicates that current LVLMs do not generalize in understanding the visual semantics of synthetic images as humans do. Our data and code are publicly available at https://github.com/GuanzhenLi/MVP-Bench.

==> body/related-work.tex <==
\section{Related Work}
% Yuxi: how multi-level visual perception is defined and constructed in our benchmark
\paragraph{Visual Perception.} 
Visual Perception represents how the human brain transforms the pattern of information on the retina into a meaningful perception of the world \cite{DEWIT2012665,cornsweet2012visual}. 
This process involves interactions among sensory and cognitive processes across hierarchical levels in the brain \cite{gordon2019intermodulation,ROUW1997209}. 
Low-level visual features refer to the properties like colors and spatial attributes, while high-level visual processing integrates with human cognitive functions (\textit{e.g.} commonsense knowledge, personal experiences) related to  recognized objects \cite{akcelik2022influence,wu2023q,1180642113,SCHINDLER202114}. 
Both perception competences are crucial, as human visual perception begins with grasping the image's main idea at a high level, and then delving into low-level features motivated by particular intentions \cite{garner1987metacognition}. 
In \dataset{}, we define five high-level categories and thirteen low-level categories. The mapping relationships between levels indicate that certain low-level features can support the high-level perception (illustrated in Section~\ref{3}).

% Yuxi: MMBench/MME - perception (coarse/fine-grained); main difference compared to ours: individually evaluate v.s. systematically diagnose
% Yuxi: multi-level perception & systematically diagnostic suite 
\paragraph{Vision--Language Benchmarks.} 
% Recently, a collection of benchmarks have been developed to evaluate MLLMs from various dimensions, such as instruction-following ability \cite{bitton2023visit,li2023m}, hallucination analysis \cite{liu2023hallusionbench,li2023evaluating}, and visual understanding \cite{schwenk2022okvqa,lu2022learn}. 
Some recent benchmarks contain visual perception as a section, but their aim to offer a comprehensive evaluation of LVLMs' various capabilities leads to an inadequate exploration of visual perception. MMBench \cite{liu2023mmbench} and MME \cite{fu2024mme} categorize visual perception based on question granularity. Although coarse perception questions are general, their questions like \textit{Counting} or \textit{Existence Detection} cannot reflect an image's main idea as high-level visual perception. Additionally, they evaluate different categories of visual perception individually, making it unavailable to compare an LVLM's different perceptions.
II-Bench\cite{liu2024ii} and DEEPEVAL\cite{yang2024can} focus on understanding deep image semantics, requiring LVLMs to perform complex commonsense reasoning based on low-level details. While they also reveal LVLMs' performance gaps across levels, these gaps are primarily due to limited reasoning abilities rather than intuitive visual perception.
The definition of perception in PCA-Bench \cite{chen2024pca} resembles our benchmark, emphasizing how perception offers a guiding context in decision-making domains. However, their images depicting environments normally do not require significant high-level perception.
\dataset{} systematically evaluates LVLMs' multi-level visual perception, with each image accompanied by high- and low-level questions simultaneously. As perceptions related to humans normally require significant perception at both levels (such as misinformation understanding or emotion recognition) \cite{peng2023agenda,thomson2022visual}, we construct image pairs containing humans to ensure that the cases can assess LVLMs' multi-level perception.

% Yuxi: also consider works on ``manipulation'': including eval (Whoops, EMU) & training (data augmentation/inflation); manipulation tools (human annotators, diffusion models, other tools)
\paragraph{Synthetic Images.} 
Recent advancements in image generation tools \cite{ramesh2021zero,rombach2021highresolution} and image editing models \cite{brooks2023instructpix2pix,zhang2023sine} have led to synthetic datasets for different tasks, such as Whoops \cite{bitton2023breaking} and StableRep \cite{tian2024stablerep}. In the process of utilizing text-to-image tools for generating synthetic images, a prompt aligned with the expected image content is essential. In previous works, the source of such prompts can be manually-crafted prompts \cite{bitton2023breaking}, text annotations in existing datasets \cite{tian2024stablerep} or prompts generated by LLMs \cite{aboutalebi2024magid,li2023stablellava,wu2023visual}. 
In \dataset{}, we generate manipulated images for constructing image pairs. To obtain a prompt tailored to each case while minimizing human effort, we employ ChatGPT to generate the prompts (\textit{cf.} Section~\ref{4.1}).

==> to_do_list.tex <==
1. The bond in Fig. 1; ticked
2. Fig. 3 (b);  ticked
3. 4.1 Step-3 Annotator agreement; ticked
4. 4.2 Distribution shift; ticked
5. Appendix: Human performance (4.2); ticked
6. Appendix: Specific Template;
7. Footnote on Page 8; ticked ??? Ask
8. Two references; ticked
